Rosita: Towards Automatic Elimination of Power-Analysis Leakage in Ciphers

Since their introduction over two decades ago, side-channel attacks have presented a serious security threat. While many ciphers' implementations employ masking techniques to protect against such attacks, they often leak secret information due to unintended interactions in the hardware. We present Rosita, a code rewrite engine that uses a leakage emulator which we amend to correctly emulate the micro-architecture of a target system. We use Rosita to automatically protect masked implementations of AES, ChaCha, and Xoodoo. For AES and Xoodoo, we show the absence of observable leakage at 1,000,000 traces with less than 21% penalty to the performance. For ChaCha, which has significantly more leakage, Rosita eliminates over 99% of the leakage, at a performance cost of 64%.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

.PHONY: all

BIBDIR     ?= /home/disy/lib/BibTeX:../../../bibtex:../bibtex
LaTeXEnv   = TEXINPUTS=".:/home/disy/lib/TeX:/home/disy/lib/ps:${TEXINPUTS}:"
BibTexEnv  = BIBINPUTS=".:${BIBDIR}:${BIBINPUTS}:"
BibFiles   = defs-abbrev,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
RmCR       = tr -d '\r'
sed        = $(shell which sed)
#PdfView    = open -a preview
#PdfView    = acroread 
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
Targets    = noleaks
SRCS = noleaks.tex # methodology.tex


# CONFIGURATION OPTIONS
# =====================

# For ACM SIG camera ready submission. This will only work if Target
# is a single identifier. You should then be able to use the "camera" target,
# after setting CamRoot appropriately. Answer "no" for re-making references.bib
# Set CamRoot as the filename root per publisher's instructions.
# Should be <paperno>-<lastname-of-first-author>
CamRoot    = <paperno>-<last>
CamDir	   = cameraready

# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Gnuplot_Sources = $(wildcard figures/*.gnuplot)
Figures = ./diagrams/dut_probing.pdf $(Gnuplot_Sources:.gnuplot=.pdf)



Pdf = $(addsuffix .pdf, $(Targets))
Tex = $(addsuffix .tex, $(Targets))
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)

%.pdf: %.perf tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

#%.eps: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

#%.pdf: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.idx *.out *.ps *-diff.* *.mps .log *.diff noleaks.pdf

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo "Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)"


##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '


noleaks.pdf: noleaks.tex  $(Figures) Makefile ${SRCS}
	${Q}if ! test -e noleaks.bbl || test noleaks.bib -nt noleaks.bbl; then rm -f noleaks.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) noleaks.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) noleaks.log ; then echo "====> BibTex" && ( $(BibTeX) noleaks > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) noleaks.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) noleaks.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) noleaks.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) noleaks.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if [ -a .NeedGS ]; then gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $@; mv tmp.pdf $@; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) noleaks.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" noleaks.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done

usb.pdf: dtrt.sty


==> gnuplot-lua-tikz-common.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%     Common style file for TeX, LaTeX and ConTeXt
%%  
%%  It is associated with the 'gnuplot.lua' script, and usually generated
%%  automatically. So take care whenever you make any changes!
%%

% check for the correct TikZ version
\def\gpchecktikzversion#1.#2\relax{%
\ifnum#1<2%
  \errmessage{PGF/TikZ version >= 2.0 is required!}%
\fi}
\expandafter\gpchecktikzversion\pgfversion\relax

% FIXME: is there a more elegant way to determine the output format?

\def\pgfsysdriver@a{pgfsys-dvi.def}       % ps
\def\pgfsysdriver@b{pgfsys-dvipdfm.def}   % pdf
\def\pgfsysdriver@c{pgfsys-dvipdfmx.def}  % pdf
\def\pgfsysdriver@d{pgfsys-dvips.def}     % ps
\def\pgfsysdriver@e{pgfsys-pdftex.def}    % pdf
\def\pgfsysdriver@f{pgfsys-tex4ht.def}    % html
\def\pgfsysdriver@g{pgfsys-textures.def}  % ps
\def\pgfsysdriver@h{pgfsys-vtex.def}      % ps
\def\pgfsysdriver@i{pgfsys-xetex.def}     % pdf

\newif\ifgppdfout\gppdfoutfalse
\newif\ifgppsout\gppsoutfalse

\ifx\pgfsysdriver\pgfsysdriver@a
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@b
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@c
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@d
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@e
  \gppdfouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@f
  % tex4ht
\else\ifx\pgfsysdriver\pgfsysdriver@g
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@h
  \gppsouttrue
\else\ifx\pgfsysdriver\pgfsysdriver@i
  \gppdfouttrue
\fi\fi\fi\fi\fi\fi\fi\fi\fi

% uncomment the following lines to make font values "appendable"
% and if you are really sure about that ;-)
% \pgfkeyslet{/tikz/font/.@cmd}{\undefined}
% \tikzset{font/.initial={}}
% \def\tikz@textfont{\pgfkeysvalueof{/tikz/font}}

%
% image related stuff
%
\def\gp@rawimage@pdf#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{/CMYK}%
  \else%
    \def\gp@temp{/RGB}%
  \fi%
  \pgf@sys@bp{#4}\pgfsysprotocol@literalbuffered{0 0}\pgf@sys@bp{#5}%
  \pgfsysprotocol@literalbuffered{0 0 cm}%
  \pgfsysprotocol@literalbuffered{BI /W #2 /H #3 /CS \gp@temp}%
  \pgfsysprotocol@literalbuffered{/BPC 8 /F /AHx ID}%
  \pgfsysprotocol@literal{#6 > EI}%
}
\def\gp@rawimage@ps#1#2#3#4#5#6{%
  \def\gp@tempa{cmyk}%
  \def\gp@tempb{#1}%
  \ifx\gp@tempa\gp@tempb%
    \def\gp@temp{4}%
  \else%
    \def\gp@temp{3}%
  \fi%
  \pgfsysprotocol@literalbuffered{0 0 translate}%
  \pgf@sys@bp{#4}\pgf@sys@bp{#5}\pgfsysprotocol@literalbuffered{scale}%
  \pgfsysprotocol@literalbuffered{#2 #3 8 [#2 0 0 -#3 0 #3]}%
  \pgfsysprotocol@literalbuffered{currentfile /ASCIIHexDecode filter}%
  \pgfsysprotocol@literalbuffered{false \gp@temp\space colorimage}%
  \pgfsysprotocol@literal{#6 >}%
}
\def\gp@rawimage@html#1#2#3#4#5#6{%
% FIXME: print a warning message here
}

\ifgppdfout
  \def\gp@rawimage{\gp@rawimage@pdf}
\else
  \ifgppsout
    \def\gp@rawimage{\gp@rawimage@ps}
  \else
    \def\gp@rawimage{\gp@rawimage@html}
  \fi
\fi


\def\gploadimage#1#2#3#4#5{%
  \pgftext[left,bottom,x=#1cm,y=#2cm] {\pgfimage[interpolate=false,width=#3cm,height=#4cm]{#5}};%
}

\def\gp@set@size#1{%
  \def\gp@image@size{#1}%
}

\def\gp@rawimage@#1#2#3#4#5#6#7#8{
  \tikz@scan@one@point\gp@set@size(#6,#7)\relax%
  \tikz@scan@one@point\pgftransformshift(#2,#3)\relax%
  \pgftext {%
    \pgfsys@beginpurepicture%
    \gp@image@size% fill \pgf@x and \pgf@y
    \gp@rawimage{#1}{#4}{#5}{\pgf@x}{\pgf@y}{#8}%
    \pgfsys@endpurepicture%
  }%
}

%% \gprawimage{color model}{xcoord}{ycoord}{# of xpixel}{# of ypixel}{xsize}{ysize}{rgb/cmyk hex data RRGGBB/CCMMYYKK ...}{file name}
%% color model is 'cmyk' or 'rgb' (default)
\def\gprawimage#1#2#3#4#5#6#7#8#9{%
  \ifx&#9&%
    \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
  \else
    \ifgppsout
      \gp@rawimage@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}
    \else
      \gploadimage{#2}{#3}{#6}{#7}{#9}
    \fi
  \fi
}

%
% gnuplottex comapatibility
% (see http://www.ctan.org/tex-archive/help/Catalogue/entries/gnuplottex.html)
%

\def\gnuplottexextension@lua{\string tex}
\def\gnuplottexextension@tikz{\string tex}

%
% gnuplot variables getter and setter
%

\def\gpsetvar#1#2{%
  \expandafter\xdef\csname gp@var@#1\endcsname{#2}
}

\def\gpgetvar#1{%
  \csname gp@var@#1\endcsname %
}

%
% some wrapper code
%

% short for a filled path
\def\gpfill#1{\path[line width=0.1\gpbaselw,draw,fill,#1]}

% short for changing the line width
\def\gpsetlinewidth#1{\pgfsetlinewidth{#1\gpbaselw}}

% short for changing the line type
\def\gpsetlinetype#1{\tikzset{gp path/.style={#1,#1 add}}}

% short for changing the dash pattern
\def\gpsetdashtype#1{\tikzset{gp path/.append style={#1}}}

% short for changing the point size
\def\gpsetpointsize#1{\tikzset{gp point/.style={mark size=#1\gpbasems}}}

% wrapper for color settings
\def\gpcolor#1{\tikzset{global #1}}
\tikzset{rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\tikzset{color=.}}}
\tikzset{global rgb color/.code={\pgfutil@definecolor{.}{rgb}{#1}\pgfutil@color{.}}}
\tikzset{global color/.code={\pgfutil@color{#1}}}

% prevent plot mark distortions due to changes in the PGF transformation matrix
% use `\gpscalepointstrue' and `\gpscalepointsfalse' for enabling and disabling
% point scaling
%
\newif\ifgpscalepoints
\tikzset{gp shift only/.style={%
  \ifgpscalepoints\else shift only\fi%
}}
\def\gppoint#1#2{%
  \path[solid] plot[only marks,gp point,mark options={gp shift only},#1] coordinates {#2};%
}


%
% char size calculation, that might be used with gnuplottex
%
% Example code (needs gnuplottex.sty):
%
%    % calculate the char size when the "gnuplot" style is used
%    \tikzset{gnuplot/.append style={execute at begin picture=\gpcalccharsize}}
%
%    \tikzset{gnuplot/.append style={font=\ttfamily\footnotesize}}
%
%    \begin{tikzpicture}[gnuplot]
%      \begin{gnuplot}[terminal=lua,%
%          terminaloptions={tikz solid nopic charsize \the\gphcharsize,\the\gpvcharsize}]
%        test
%      \end{gnuplot}
%    \end{tikzpicture}
%
%%%
% The `\gpcalccharsize' command fills the lengths \gpvcharsize and \gphcharsize with
% the values of the current default font used within nodes and is meant to be called
% within a tikzpicture environment.
% 
\newdimen\gpvcharsize
\newdimen\gphcharsize
\def\gpcalccharsize{%
  \pgfinterruptboundingbox%
  \pgfsys@begininvisible%
  \node at (0,0) {%
    \global\gphcharsize=1.05\fontcharwd\font`0%
    \global\gpvcharsize=1.05\fontcharht\font`0%
    \global\advance\gpvcharsize by 1.05\fontchardp\font`g%
  };%
  \pgfsys@endinvisible%
  \endpgfinterruptboundingbox%
}

%
%  define a rectangular node in tikz e.g. for the plot area
%
%  #1 node name
%  #2 coordinate of "south west"
%  #3 coordinate of "north east"
%
\def\gpdefrectangularnode#1#2#3{%
  \expandafter\gdef\csname pgf@sh@ns@#1\endcsname{rectangle}
  \expandafter\gdef\csname pgf@sh@np@#1\endcsname{%
    \def\southwest{#2}%
    \def\northeast{#3}%
  }
  \pgfgettransform\pgf@temp%
  % once it is defined, no more transformations will be applied, I hope
  \expandafter\xdef\csname pgf@sh@nt@#1\endcsname{\pgf@temp}%
  \expandafter\xdef\csname pgf@sh@pi@#1\endcsname{\pgfpictureid}%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  You may want to adapt the following to fit your needs (in your 
%%  individual style file and/or within your document).
%%

%
% style for every plot
%
\tikzset{gnuplot/.style={%
  >=stealth',%
  line cap=round,%
  line join=round,%
}}

\tikzset{gp node left/.style={anchor=mid west,yshift=-.12ex}}
\tikzset{gp node center/.style={anchor=mid,yshift=-.12ex}}
\tikzset{gp node right/.style={anchor=mid east,yshift=-.12ex}}

% basic plot mark size (points)
\newdimen\gpbasems
\gpbasems=.4pt

% basic linewidth
\newdimen\gpbaselw
\gpbaselw=.4pt

% this is the default color for pattern backgrounds
\colorlet{gpbgfillcolor}{white}

% set background color and fill color
\def\gpsetbgcolor#1{%
  \pgfutil@definecolor{gpbgfillcolor}{rgb}{#1}%
  \tikzset{tight background,background rectangle/.style={fill=gpbgfillcolor},show background rectangle}%
}

% this should reverse the normal text node presets, for the
% later referencing as described below
\tikzset{gp refnode/.style={coordinate,yshift=.12ex}}

% to add an empty label with the referenceable name "my node"
% to the plot, just add the following line to your gnuplot
% file:
%
% set label "" at 1,1 font ",gp refnode,name=my node"
%

% enlargement of the bounding box in standalone mode (only used by LaTeX/ConTeXt)
\def\gpbboxborder{0mm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  The following TikZ-styles are derived from the 'pgf.styles.*' tables
%%  in the Lua script.
%%  To change the number of used styles you should change them there and
%%  regenerate this style file.
%%

% arrow styles settings
\tikzset{gp arrow 1/.style={>=latex}}
\tikzset{gp arrow 2/.style={>=angle 90}}
\tikzset{gp arrow 3/.style={>=angle 60}}
\tikzset{gp arrow 4/.style={>=angle 45}}
\tikzset{gp arrow 5/.style={>=o}}
\tikzset{gp arrow 6/.style={>=*}}
\tikzset{gp arrow 7/.style={>=diamond}}
\tikzset{gp arrow 8/.style={>=open diamond}}
\tikzset{gp arrow 9/.style={>={]}}}
\tikzset{gp arrow 10/.style={>={[}}}
\tikzset{gp arrow 11/.style={>=)}}
\tikzset{gp arrow 12/.style={>=(}}

% plotmark settings
\tikzset{gp mark 0/.style={mark size=.5\pgflinewidth,mark=*}}
\tikzset{gp mark 1/.style={mark=+}}
\tikzset{gp mark 2/.style={mark=x}}
\tikzset{gp mark 3/.style={mark=star}}
\tikzset{gp mark 4/.style={mark=square}}
\tikzset{gp mark 5/.style={mark=square*}}
\tikzset{gp mark 6/.style={mark=o}}
\tikzset{gp mark 7/.style={mark=*}}
\tikzset{gp mark 8/.style={mark=triangle}}
\tikzset{gp mark 9/.style={mark=triangle*}}
\tikzset{gp mark 10/.style={mark=triangle,every mark/.append style={rotate=180}}}
\tikzset{gp mark 11/.style={mark=triangle*,every mark/.append style={rotate=180}}}
\tikzset{gp mark 12/.style={mark=diamond}}
\tikzset{gp mark 13/.style={mark=diamond*}}
\tikzset{gp mark 14/.style={mark=otimes}}
\tikzset{gp mark 15/.style={mark=oplus}}

% pattern settings
\tikzset{gp pattern 0/.style={white}}
\tikzset{gp pattern 1/.style={pattern=north east lines}}
\tikzset{gp pattern 2/.style={pattern=north west lines}}
\tikzset{gp pattern 3/.style={pattern=crosshatch}}
\tikzset{gp pattern 4/.style={pattern=grid}}
\tikzset{gp pattern 5/.style={pattern=vertical lines}}
\tikzset{gp pattern 6/.style={pattern=horizontal lines}}
\tikzset{gp pattern 7/.style={pattern=dots}}
\tikzset{gp pattern 8/.style={pattern=crosshatch dots}}
\tikzset{gp pattern 9/.style={pattern=fivepointed stars}}
\tikzset{gp pattern 10/.style={pattern=sixpointed stars}}
\tikzset{gp pattern 11/.style={pattern=bricks}}

% if the 'tikzplot' option is used the corresponding lines will be smoothed by default
\tikzset{gp plot axes/.style=}
\tikzset{gp plot border/.style=}
\tikzset{gp plot 0/.style=smooth}
\tikzset{gp plot 1/.style=smooth}
\tikzset{gp plot 2/.style=smooth}
\tikzset{gp plot 3/.style=smooth}
\tikzset{gp plot 4/.style=smooth}
\tikzset{gp plot 5/.style=smooth}
\tikzset{gp plot 6/.style=smooth}
\tikzset{gp plot 7/.style=smooth}

% linestyle settings
\tikzset{gp lt axes/.style=dotted}
\tikzset{gp lt border/.style=solid}

% linestyle "addon" settings for overwriting a default linestyle within the
% TeX document via eg. \tikzset{gp lt plot 1 add/.style={fill=black,draw=none}} etc.
\tikzset{gp lt axes add/.style={}}
\tikzset{gp lt border add/.style={}}
\tikzset{gp lt plot 0 add/.style={}}
\tikzset{gp lt plot 1 add/.style={}}
\tikzset{gp lt plot 2 add/.style={}}
\tikzset{gp lt plot 3 add/.style={}}
\tikzset{gp lt plot 4 add/.style={}}
\tikzset{gp lt plot 5 add/.style={}}
\tikzset{gp lt plot 6 add/.style={}}
\tikzset{gp lt plot 7 add/.style={}}
\tikzset{gp lt plot 0/.style={}}
\tikzset{gp lt plot 1/.style={}}
\tikzset{gp lt plot 2/.style={}}
\tikzset{gp lt plot 3/.style={}}
\tikzset{gp lt plot 4/.style={}}
\tikzset{gp lt plot 5/.style={}}
\tikzset{gp lt plot 6/.style={}}
\tikzset{gp lt plot 7/.style={}}

% linestyle color settings
\colorlet{gp lt color axes}{black!30}
\colorlet{gp lt color border}{black}

% dash type settings
% Define this as a macro so that the dash patterns expand later with the current \pgflinewidth.
\def\gpdashlength{\pgflinewidth}
\tikzset{gp dt 0/.style={solid}}
\tikzset{gp dt 1/.style={solid}}
\tikzset{gp dt 2/.style={dash pattern=on 7.5*\gpdashlength off 7.5*\gpdashlength}}
\tikzset{gp dt 3/.style={dash pattern=on 3.75*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 4/.style={dash pattern=on 1*\gpdashlength off 2.8125*\gpdashlength}}
\tikzset{gp dt 5/.style={dash pattern=on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt 6/.style={dash pattern=on 5.625*\gpdashlength off 5.625*\gpdashlength on 1*\gpdashlength off 5.625*\gpdashlength}}
\tikzset{gp dt 7/.style={dash pattern=on 3.75*\gpdashlength off 3.75*\gpdashlength on 3.75*\gpdashlength off 11.25*\gpdashlength}}
\tikzset{gp dt 8/.style={dash pattern=on 1*\gpdashlength off 3.75*\gpdashlength on 11.25*\gpdashlength off 3.75*\gpdashlength on 1*\gpdashlength off 3.75*\gpdashlength}}
\tikzset{gp dt solid/.style={solid}}
\tikzset{gp dt axes/.style={dotted}}

% command for switching to colored lines
\def\gpcoloredlines{%
  \colorlet{gp lt color 0}{red}%
  \colorlet{gp lt color 1}{green}%
  \colorlet{gp lt color 2}{blue}%
  \colorlet{gp lt color 3}{magenta}%
  \colorlet{gp lt color 4}{cyan}%
  \colorlet{gp lt color 5}{yellow}%
  \colorlet{gp lt color 6}{orange}%
  \colorlet{gp lt color 7}{purple}%
}

% command for switching to monochrome (black) lines
\def\gpmonochromelines{%
  \colorlet{gp lt color 0}{black}%
  \colorlet{gp lt color 1}{black}%
  \colorlet{gp lt color 2}{black}%
  \colorlet{gp lt color 3}{black}%
  \colorlet{gp lt color 4}{black}%
  \colorlet{gp lt color 5}{black}%
  \colorlet{gp lt color 6}{black}%
  \colorlet{gp lt color 7}{black}%
}

%
% some initialisations
%
% by default all lines will be colored
\gpcoloredlines
\gpsetpointsize{4}
\gpsetlinetype{gp lt solid}
\gpscalepointsfalse
\endinput


==> gnuplot-lua-tikz.tex <==
%%
%%  plain TeX wrapper for gnuplot-tikz style file
%%
\input tikz.tex
\usetikzlibrary{arrows,patterns,plotmarks,backgrounds}

\edef\tikzatcode{\the\catcode`\@}
\catcode`\@=11

\input gnuplot-lua-tikz-common.tex


\catcode`\@=\tikzatcode

\endinput


==> plots/Makefile <==
SRC=./src
B=./src/build
BS=./src/buildsmall
DATA=./data
TVALS_DATA=tvals_signed.txt
TVALS_GPSCRIPT=plot_tvals_signed
MERGED_LIST=
#MERGED_LIST= \
	f030_xoodoo_check_merged_10k.pdf 
#f030_xoodoo_fixed_10k_nocycles.pdf \
#
all: elmo_ldr-ldr-check_10k.pdf \
	elmo-ori_ldr-ldr-check_10k.pdf \
	elmo_sr_check_10k.pdf \
	f030_sr_check_10k.pdf \
	f030_aes-fixed_10k.pdf \
	f030_aes_check_10k.pdf \
	f030_sr_fixed_10k_nocycles.pdf \
	f030_sr_check_10k_nocycles.pdf \
	f030_sr_check_20k_mask_R_movs.pdf \
	f030_sr_check_20k_mask_rrrr_movs.pdf \
	f030_sr_check_10k_leaks_any.pdf \
	f030_sr_check_10k_U_removed.pdf \
	f030_ldr-ldr-check_10k.pdf \
	f030_ldr-ldr-fix_40k.pdf \
	f030_xoodoo_1_check_10k.pdf \
	f030_xoodoo_1_fixed_10k.pdf \
	f030_chacha20_1_check_10k.pdf \
	f030_chacha20_1_fixed_10k.pdf \
	f030_xoodoo_2_check_10k.pdf \
	f030_xoodoo_2_fixed_10k.pdf \
	f030_xoodoo_5_check_10k.pdf \
	f030_xoodoo_5_fixed_10k.pdf \
	f030_chacha20_5_check_10k.pdf \
	f030_chacha20_5_fixed_10k.pdf \
	f030_xoodoo_100other_check_10k.pdf \
	f030_xoodoo_100other_fixed_10k.pdf \
	f030_xoodoo_check_200k.pdf \
	f030_xoodoo_check_1m.pdf \
	f030_xoodoo_fixed_200k.pdf \
	f030_xoodoo_fixed_1m.pdf \
	f030_chacha20_check_1m.pdf \
	f030_chacha20_fixed_1m.pdf \
	f030_aes_1_check_10k.pdf \
	f030_aes_1_fixed_10k.pdf \
	f030_aes_2_check_10k.pdf \
	f030_aes_2_fixed_10k.pdf \
	f030_aes_5_check_10k.pdf \
	f030_aes_5_fixed_10k.pdf \
	f030_aes_check_200k.pdf \
	f030_aes_check_1m.pdf \
	f030_aes_fixed_200k.pdf \
	f030_aes_fixed_1m.pdf \
	f030_aes_100other_check_10k.pdf \
	f030_aes_100other_fixed_10k.pdf \
	f030_chacha20_100other_check_10k.pdf \
	f030_chacha20_100other_fixed_10k.pdf \
	ttest_trend.pdf \
	ttest_trend_profiled.pdf \
	traces_notaligned.pdf \
	traces_aligned.pdf \
	f030_ttest_trend_merged.pdf \
	aes_leakcount.pdf \
	xoodoo_leakcount.pdf \
	chacha20_leakcount.pdf \
	f030_str-eors_10k.pdf \
	elmo_str-eors_10k.pdf \
	f030_ldr-eors_10k.pdf \
	elmo_ldr-eors_10k.pdf \
	elmo_ori_ldr-eors_10k.pdf \
	elmo_ori_str-eors_10k.pdf \
	f030_str-eors_corr_10k.pdf \
	f030_str-eors_merge_10k.pdf \
	f030_x-eors_corr_merge.pdf \
	${MERGED_LIST}

f030_x-eors_corr_merge.pdf: ./src/plot_corr_merge ./data/f030_x-eors_corr_merge
	${B} ./src/plot_corr_merge ./data/f030_x-eors_corr_merge

f030_str-eors_merge_10k.pdf: ./src/plot_tvalsc_merge
	${B} ./src/plot_tvalsc_merge ./data/f030_str-eors_merge_10k

f030_str-eors_corr_10k.pdf: ./src/plot_corr ./src/*.gp
	${B} ./src/plot_corr ./data/f030_str-eors_corr_10k

f030_ttest_trend_merged.pdf: ./src/plot_tvals_sample_merged 
	${B} ./src/plot_tvals_sample_merged ./data/f030_ttest_trend_merged

elmo_ldr-ldr-check_10k.pdf: ./src/plot_tvalsELMO-ldr-ldr ./data/elmo_ldr-ldr-check_10k/*
	${B} ./src/plot_tvalsELMO-ldr-ldr ./data/elmo_ldr-ldr-check_10k/

elmo-ori_ldr-ldr-check_10k.pdf: ./src/plot_tvalsELMO-ldr-ldr ./data/elmo-ori_ldr-ldr-check_10k/*
	${B} ./src/plot_tvalsELMO-ldr-ldr ./data/elmo-ori_ldr-ldr-check_10k/

elmo_sr_check_10k.pdf: ./src/plot_tvalsELMO ./data/elmo_sr_check_10k/*
	${B} ./src/plot_tvalsELMO ./data/elmo_sr_check_10k

elmo_ori_ldr-eors_10k.pdf: ./src/plot_tvals ./data/elmo_ori_ldr-eors_10k/*
	${B} ./src/plot_tvalsELMOc ./data/elmo_ori_ldr-eors_10k

elmo_ori_str-eors_10k.pdf: ./src/plot_tvalsELMO ./data/elmo_ori_str-eors_10k/*
	${B} ./src/plot_tvalsELMOc ./data/elmo_ori_str-eors_10k

f030_str-eors_10k.pdf: ./src/plot_tvals ./data/f030_str-eors_10k/*
	${B} ./src/plot_tvalsc ./data/f030_str-eors_10k

elmo_str-eors_10k.pdf: ./src/plot_tvalsELMO ./data/elmo_str-eors_10k/*
	${B} ./src/plot_tvalsELMOc ./data/elmo_str-eors_10k

f030_ldr-eors_10k.pdf: ./src/plot_tvals ./data/f030_ldr-eors_10k/*
	${B} ./src/plot_tvalsc ./data/f030_ldr-eors_10k

elmo_ldr-eors_10k.pdf: ./src/plot_tvalsELMO ./data/elmo_ldr-eors_10k/*
	${B} ./src/plot_tvalsELMOc ./data/elmo_ldr-eors_10k


f030_aes-fixed_10k.pdf: ./src/plot_tvalsAES_fixed-profiled ./data/f030_aes-fixed_10k/*
	${B} ./src/plot_tvalsAES_fixed-profiled ./data/f030_aes-fixed_10k

f030_aes_check_10k.pdf: ./src/plot_tvalsAES_check ./data/f030_aes_check_10k/*
	${B} ./src/plot_tvalsAES_check ./data/f030_aes_check_10k

f030_sr_check_10k.pdf: ./src/plot_tvals ./data/f030_sr_check_10k/*
	${B} ./src/plot_tvals ./data/f030_sr_check_10k

f030_sr_fixed_10k_nocycles.pdf: ./src/plot_tvalse_40 ./data/f030_sr_fixed_10k_nocycles/*
	${B} ./src/plot_tvalse_40 ./data/f030_sr_fixed_10k_nocycles

f030_sr_check_10k_nocycles.pdf: ./src/plot_tvalse ./data/f030_sr_check_10k_nocycles/*
	${B} ./src/plot_tvalse ./data/f030_sr_check_10k_nocycles

f030_sr_check_20k_mask_R_movs.pdf: ./src/plot_tvals ./data/f030_sr_check_20k_mask_R_movs/*
	${B} ./src/plot_tvals ./data/f030_sr_check_20k_mask_R_movs

f030_sr_check_20k_mask_rrrr_movs.pdf: ./src/plot_tvals ./data/f030_sr_check_20k_mask_rrrr_movs/*
	${B} ./src/plot_tvals ./data/f030_sr_check_20k_mask_rrrr_movs

f030_sr_check_10k_leaks_any.pdf: ./src/plot_tvals ./data/f030_sr_check_10k_leaks_any/*
	${B} ./src/plot_tvals ./data/f030_sr_check_10k_leaks_any

f030_sr_check_10k_U_removed.pdf: ./src/plot_tvals ./data/f030_sr_check_10k_U_removed/*
	${B} ./src/plot_tvals ./data/f030_sr_check_10k_U_removed

f030_ldr-ldr-check_10k.pdf: ./src/plot_tvals ./data/f030_ldr-ldr-check_10k/*
	${B} ./src/plot_tvals ./data/f030_ldr-ldr-check_10k

f030_xoodoo_fixed_10k_nocycles.pdf: ./src/*.gp ./data/f030_xoodoo_fixed_10k_nocycles/*
	${B} ./data/f030_xoodoo_fixed_10k_nocycles/plot_tvals ./data/f030_xoodoo_fixed_10k_nocycles

f030_xoodoo_1_check_10k.pdf: ./src/*.gp ./data/f030_xoodoo_1_check_10k/*
	${B} ./data/f030_xoodoo_1_check_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_1_check_10k/${TVALS_DATA}

f030_xoodoo_1_fixed_10k.pdf: ./src/*.gp ./data/f030_xoodoo_1_fixed_10k/*
	${B} ./data/f030_xoodoo_1_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_1_fixed_10k/${TVALS_DATA}

f030_chacha20_1_check_10k.pdf: ./src/*.gp ./data/f030_chacha20_1_check_10k/*
	${B} ./data/f030_chacha20_1_check_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_1_check_10k/${TVALS_DATA}

f030_chacha20_1_fixed_10k.pdf: ./src/*.gp ./data/f030_chacha20_1_fixed_10k/*
	${B} ./data/f030_chacha20_1_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_1_fixed_10k/${TVALS_DATA}

f030_xoodoo_2_check_10k.pdf: ./src/*.gp ./data/f030_xoodoo_2_check_10k/*
	${B} ./data/f030_xoodoo_2_check_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_2_check_10k/${TVALS_DATA}

f030_xoodoo_2_fixed_10k.pdf: ./src/*.gp ./data/f030_xoodoo_2_fixed_10k/*
	${B} ./data/f030_xoodoo_2_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_2_fixed_10k/${TVALS_DATA}

f030_xoodoo_5_check_10k.pdf: ./src/*.gp ./data/f030_xoodoo_5_check_10k/*
	${B} ./data/f030_xoodoo_5_check_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_5_check_10k/${TVALS_DATA}

f030_xoodoo_5_fixed_10k.pdf: ./src/*.gp ./data/f030_xoodoo_5_fixed_10k/*
	${B} ./data/f030_xoodoo_5_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_5_fixed_10k/${TVALS_DATA}

f030_chacha20_5_check_10k.pdf: ./src/*.gp ./data/f030_chacha20_5_check_10k/*
	${B} ./data/f030_chacha20_5_check_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_5_check_10k/${TVALS_DATA}

f030_chacha20_5_fixed_10k.pdf: ./src/*.gp ./data/f030_chacha20_5_fixed_10k/*
	${B} ./data/f030_chacha20_5_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_5_fixed_10k/${TVALS_DATA}

f030_xoodoo_100other_check_10k.pdf: ./src/*.gp ./data/f030_xoodoo_100other_check_10k/*
	${B} ./data/f030_xoodoo_100other_check_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_100other_check_10k/${TVALS_DATA}

f030_xoodoo_100other_fixed_10k.pdf: ./src/*.gp ./data/f030_xoodoo_100other_fixed_10k/*
	${B} ./data/f030_xoodoo_100other_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_100other_fixed_10k/${TVALS_DATA}

f030_xoodoo_check_200k.pdf: ./src/*.gp ./data/f030_xoodoo_check_200k/*
	${B} ./data/f030_xoodoo_check_200k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_check_200k/${TVALS_DATA}

f030_xoodoo_check_1m.pdf: ./src/*.gp ./data/f030_xoodoo_check_1m/*
	${B} ./data/f030_xoodoo_check_1m/${TVALS_GPSCRIPT} ./data/f030_xoodoo_check_1m/${TVALS_DATA}

f030_xoodoo_fixed_200k.pdf: ./src/*.gp ./data/f030_xoodoo_fixed_200k/*
	${B} ./data/f030_xoodoo_fixed_200k/${TVALS_GPSCRIPT} ./data/f030_xoodoo_fixed_200k/${TVALS_DATA}

f030_xoodoo_fixed_1m.pdf: ./src/*.gp ./data/f030_xoodoo_fixed_1m/*
	${B} ./data/f030_xoodoo_fixed_1m/${TVALS_GPSCRIPT} ./data/f030_xoodoo_fixed_1m/${TVALS_DATA}

f030_chacha20_check_1m.pdf: ./src/*.gp ./data/f030_chacha20_check_1m/*
	${B} ./data/f030_chacha20_check_1m/${TVALS_GPSCRIPT} ./data/f030_chacha20_check_1m/${TVALS_DATA}

f030_chacha20_fixed_1m.pdf: ./src/*.gp ./data/f030_chacha20_fixed_1m/*
	${B} ./data/f030_chacha20_fixed_1m/${TVALS_GPSCRIPT} ./data/f030_chacha20_fixed_1m/${TVALS_DATA}

#f030_xoodoo_check_merged_10k.pdf: ./src/*.gp ./data/f030_xoodoo_*_check_*/*
#	paste ./data/f030_xoodoo_1_check_10k/tvals.txt \
#		./data/f030_xoodoo_2_check_10k/tvals.txt \
#		./data/f030_xoodoo_5_check_10k/tvals.txt \
#		./data/f030_xoodoo_check_200k/tvals.txt \
#		./data/f030_xoodoo_100other_check_10k/tvals.txt > ./data/f030_xoodoo_check_merged_10k/tvals.txt
#	paste ./data/f030_xoodoo_1_check_10k/tvals_signed.txt \
#		./data/f030_xoodoo_2_check_10k/tvals_signed.txt \
#		./data/f030_xoodoo_5_check_10k/tvals_signed.txt \
#		./data/f030_xoodoo_check_200k/tvals_signed.txt \
#		./data/f030_xoodoo_100other_check_10k/tvals_signed.txt > ./data/f030_xoodoo_check_merged_10k/tvals_signed.txt
#
#
#	${B} ./data/f030_xoodoo_check_merged_10k/plot_tvals ./data/f030_xoodoo_check_merged_10k

f030_aes_2_check_10k.pdf: ./src/*.gp ./data/f030_aes_2_check_10k/*
	${B} ./data/f030_aes_2_check_10k/${TVALS_GPSCRIPT} ./data/f030_aes_2_check_10k/${TVALS_DATA}

f030_aes_2_fixed_10k.pdf: ./src/*.gp ./data/f030_aes_2_fixed_10k/*
	${B} ./data/f030_aes_2_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_aes_2_fixed_10k/${TVALS_DATA}

f030_aes_1_check_10k.pdf: ./src/*.gp ./data/f030_aes_1_check_10k/*
	${B} ./data/f030_aes_1_check_10k/${TVALS_GPSCRIPT} ./data/f030_aes_1_check_10k/${TVALS_DATA}

f030_aes_1_fixed_10k.pdf: ./src/*.gp ./data/f030_aes_1_fixed_10k/*
	${B} ./data/f030_aes_1_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_aes_1_fixed_10k/${TVALS_DATA}

f030_aes_5_check_10k.pdf: ./src/*.gp ./data/f030_aes_5_check_10k/*
	${B} ./data/f030_aes_5_check_10k/${TVALS_GPSCRIPT} ./data/f030_aes_5_check_10k/${TVALS_DATA}

f030_aes_5_fixed_10k.pdf: ./src/*.gp ./data/f030_aes_5_fixed_10k/*
	${B} ./data/f030_aes_5_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_aes_5_fixed_10k/${TVALS_DATA}

f030_aes_check_200k.pdf: ./src/*.gp ./data/f030_aes_check_200k/*
	${B} ./data/f030_aes_check_200k/${TVALS_GPSCRIPT} ./data/f030_aes_check_200k/${TVALS_DATA}

f030_aes_check_1m.pdf: ./src/*.gp ./data/f030_aes_check_1m/*
	${B} ./data/f030_aes_check_1m/${TVALS_GPSCRIPT} ./data/f030_aes_check_1m/${TVALS_DATA}

f030_aes_fixed_200k.pdf: ./src/*.gp ./data/f030_aes_fixed_200k/*
	${B} ./data/f030_aes_fixed_200k/${TVALS_GPSCRIPT} ./data/f030_aes_fixed_200k/${TVALS_DATA}

f030_aes_fixed_1m.pdf: ./src/*.gp ./data/f030_aes_fixed_1m/*
	${B} ./data/f030_aes_fixed_1m/${TVALS_GPSCRIPT} ./data/f030_aes_fixed_1m/${TVALS_DATA}

f030_aes_100other_check_10k.pdf: ./src/*.gp ./data/f030_aes_100other_check_10k/*
	${B} ./data/f030_aes_100other_check_10k/${TVALS_GPSCRIPT} ./data/f030_aes_100other_check_10k/${TVALS_DATA}

f030_aes_100other_fixed_10k.pdf: ./src/*.gp ./data/f030_aes_100other_fixed_10k/*
	${B} ./data/f030_aes_100other_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_aes_100other_fixed_10k/${TVALS_DATA}

f030_chacha20_100other_check_10k.pdf: ./src/*.gp ./data/f030_chacha20_100other_check_10k/*
	${B} ./data/f030_chacha20_100other_check_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_100other_check_10k/${TVALS_DATA}

f030_chacha20_100other_fixed_10k.pdf: ./src/*.gp ./data/f030_chacha20_100other_fixed_10k/*
	${B} ./data/f030_chacha20_100other_fixed_10k/${TVALS_GPSCRIPT} ./data/f030_chacha20_100other_fixed_10k/${TVALS_DATA}

f030_ldr-ldr-fix_40k.pdf: ./src/plot_tvals ./data/f030_ldr-ldr-fix_40k/*
	${B} ./src/plot_tvals ./data/f030_ldr-ldr-fix_40k

ttest_trend.pdf: ./src/plot_trend ./data/ttest_trend/*
	${B} ./src/plot_trend ./data/ttest_trend

ttest_trend_profiled.pdf: ./src/plot_trend ./data/ttest_trend_profiled/*
	${B} ./src/plot_trend ./data/ttest_trend_profiled

traces_notaligned.pdf: ./src/plot_traces_notaligned ./data/traces_notaligned/*
	${B} ./src/plot_traces_notaligned ./data/traces_notaligned

traces_aligned.pdf: ./src/plot_traces_aligned ./data/traces_aligned/*
	${B} ./src/plot_traces_aligned ./data/traces_aligned

aes_leakcount.pdf: ./data/aes_leakcount/*
	${BS} ./data/aes_leakcount/plot_average ./data/aes_leakcount/

xoodoo_leakcount.pdf: ./data/xoodoo_leakcount/*
	${BS} ./data/xoodoo_leakcount/plot_average ./data/xoodoo_leakcount/

chacha20_leakcount.pdf: ./data/chacha20_leakcount/*
	${BS} ./data/chacha20_leakcount/plot_average ./data/chacha20_leakcount/

lean:
	rm *.pdf


==> plots/data/aes_leakcount/plot_average <==
set key bottom right

stats './data/aes_leakcount/caverage_all.txt'  using 1:2 nooutput
set yrange [0:80]
set xrange [0:100]
set ytics 40
set style data boxplot
set errorbars 1.0
set style fill transparent solid 1.0 noborder
set xlabel "Number of Inputs"
set ylabel "Number of Leaks"
plot   './data/aes_leakcount/caverage_all.txt' using ($0+0.5):2:(0.5):($1-$3) with boxxyerror fillcolor "grey" t "95% confidence interval", \
       './data/aes_leakcount/caverage_all.txt' using 0:2 with steps linecolor "red" t "Average"\



==> plots/data/chacha20_leakcount/plot_average <==
set key bottom right

stats './data/chacha20_leakcount/caverage_all.txt'  using 1:2 nooutput
set yrange [0:300]
set xrange [0:100]
set ytics 100
set style data boxplot
set errorbars 1.0
set style fill transparent solid 1.0 noborder
set xlabel "Number of Inputs"
set ylabel "Number of Leaks"
plot   './data/chacha20_leakcount/caverage_all.txt' using ($0+0.5):2:(0.5):($1-$3) with boxxyerror fillcolor "grey" t "95% confidence interval", \
       './data/chacha20_leakcount/caverage_all.txt' using 0:2 with steps linecolor "red" t "Average"\



==> plots/data/f030_xoodoo_check_merged_10k/plot_tvals <==
set key bottom right
set yrange [-15:15]
set ytics 5

C = 9.765625
#C=1
F = word(FILES,1)

load 'xoodoo_xrange.gp'
load 'threshold.gp'
load 'style_tvals.gp'
set xlabel "Cycle"
set ylabel "{/:Italic t}-test value"
plot for [FILE in FILES] FILE using ($0/C):4 with lines ls 1 lc rgb "#00000000" t "", \
     for [FILE in FILES] FILE using ($0/C):3 with lines ls 1 lc rgb "#00FF4444" t "", \
     for [FILE in FILES] FILE using ($0/C):2 with lines ls 1 lc rgb "#008888FF" t "", \
     for [FILE in FILES] FILE using ($0/C):1 with lines ls 1 lc rgb "#00AAFFAA" t "" 


==> plots/data/xoodoo_leakcount/plot_average <==
set key bottom right

stats './data/xoodoo_leakcount/caverage_all.txt'  using 1:2 nooutput
set yrange [0:80]
set xrange [0:100]
set ytics 40
set style data boxplot
set errorbars 1.0
set style fill transparent solid 1.0 noborder
set xlabel "Number of Inputs"
set ylabel "Number of Leaks"
plot   './data/xoodoo_leakcount/caverage_all.txt' using ($0+0.5):2:(0.5):($1-$3) with boxxyerror fillcolor "grey" t "95% confidence interval", \
       './data/xoodoo_leakcount/caverage_all.txt' using 0:2 with steps linecolor "red" t "Average"\



==> plots/src/aes_plot_tvals_sample_merged <==

set yrange [0:80]
set xtics 0, 50000, 200000
#set xrange [0:10]
#set xtics ("0" 0, "2k" 20, "4k" 40, "6k" 60, "8k" 80, "10k" 100, "12k" 120, "14k" 140)
#set xtics ("0" 0, "2k" 200, "4k" 400, "6k" 600, "8k" 800, "10k" 1000, "12k" 1200, "14k" 1400, "16k" 1600, "18k" 1800, "20k" 2000)
#
set format x "%2.0s%c"
set label "Original AES implementation" at 10000,70
set arrow 3 from 90000,66 to 110000,60 head

set label "Fixed AES implementation" at 24500,20
set arrow 2 from 27000,15 to 10000,4 head

set arrow 1 from graph 0, first 4.5 to graph 1, first 4.5 nohead
set arrow 1 lc rgb "red"
set arrow 1 filled
set arrow 1 front 

set xlabel "Trace count"
set ylabel "Max {/:Italic t}-test value"



plot for [FILE in FILES] sprintf('%s/../f030_ttest_trend_aes-check_200k/tvals_sample.txt',FILE)  using ($0 * 2500):1 with linespoints ps .01 lc "#00CC00" lw 1 t "" , \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_aes-fixed_200k/tvals_sample.txt',FILE)  using ($0 * 2500):1 with linespoints ps .01 lc "#0000FF"  lw 1 t ""


==> plots/src/plot_corr_merge <==

set key font ',8'
set key top left
set key on
set key Right 

set ytics 0.05
set yrange [-0.2:0.2]
set xrange [0:40]
F = word(FILES,1)
#set samples 1000
C=9.76
load 'threshold.gp'
set xlabel "Cycle"
set ylabel "Pearson Coefficient"

plot for [FILE in FILES] sprintf('%s/../f030_str-eors_corr_10k/corr.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#2222FF' t "str - eors", \
  for [FILE in FILES] sprintf('%s/../f030_ldr-eors_corr_10k/corr.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#FF2222' t "ldr - eors"


==> plots/src/plot_trend <==
set yrange [-0.3:]
set ylabel "Newly discovered\nleaks"
set xlabel "Run number"
set xtics 1, 2
plot sprintf('%s/data.txt',FILES) using 0:1 with linespoints ps .1  t ''


==> plots/src/plot_tvalsELMO-ldr-ldr <==

set key bottom right
set yrange [-15:15]
set ytics 5

C = 9.765625
#C=1
F = word(FILES,1)
X_MAX = real(system(sprintf("tail -n 1 %s/cycles.txt  | cut -d ' ' -f1",F)))/C
set xrange [0:X_MAX]

load 'threshold.gp'
set xlabel "Cycle"
set ylabel "{/:Italic t}-test value"
plot for [FILE in FILES] sprintf('%s/cycles.txt',FILE) using ($1/C):2:3:4 with vectors nohead ls 1 lc 'grey' notitle , \
    for [FILE in FILES] sprintf('%s/tvals.txt',FILE) using ($0):1 with lines lt 1 lc rgb '#226622' t "" 



==> plots/src/plot_tvalsELMOc <==

set key bottom right
set yrange [-15:15]
set ytics 5

#C = 9.765625
C=1
F = word(FILES,1)
X_MAX = real(system(sprintf("tail -n 1 %s/cycles.txt  | cut -d ' ' -f1",F)))/C
set xrange [0:X_MAX]

load 'threshold.gp'
set xlabel "Cycle"
set ylabel "{/:Italic t}-test value"
plot for [FILE in FILES] sprintf('%s/cycles.txt',FILE) using ($1/C):2:3:4 with vectors nohead ls 1 lc 'grey' notitle , \
    for [FILE in FILES] sprintf('%s/tvals.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#226622' t "" 



==> plots/src/plot_tvals_sample_merged <==
set key font ",8"
set key on inside right top horizontal spacing 1 width 0.1
set yrange [0:150]
set xtics 20000, 100000, 800000
set xrange [20000:800000]
set format x "%2.0s%c" 

set arrow 1 from graph 0, first 4.5 to graph 1, first 4.5 nohead
set arrow 1 lc rgb "red"
set arrow 1 filled
set arrow 1 back 

set xlabel "Trace count"
set ylabel "Max {/:Italic t}-test value"
SCALE=20000

plot for [FILE in FILES] sprintf('%s/../f030_ttest_trend_aes-check_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints dt 9 ps .01 lc "#3333FF" lw 1 t "AES Original" , \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_aes-fixed_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints ps .01 lc "#3333FF"  lw 1 t "AES Fixed", \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_xoodoo-check_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints dt 9 ps .01 lc "#33CC33"  lw 1 t "Xoodoo Original", \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_xoodoo-fixed_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints ps .01 lc "#33CC33"  lw 1 t "Xoodoo Fixed", \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_chacha20-check_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints dt 9 ps .01 lc "#CC33CC"  lw 1 t "Chacha20 Original", \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_chacha20-fixed_1m/tvals_sample.txt',FILE)  using ($0 * SCALE):1 with linespoints ps .01 lc "#CC33CC"  lw 1 t "Chacha20 Fixed"


==> plots/src/plot_tvalsc <==
set key bottom right
set yrange [-15:15]
set ytics 5

C = 9.765625
#C=1
F = word(FILES,1)
X_MAX = real(system(sprintf("tail -n 1 %s/cycles.txt  | cut -d ' ' -f1",F)))
set xrange [0:X_MAX]

load 'threshold.gp'
set xlabel "Cycle"
set ylabel "{/:Italic t}-test value"
plot for [FILE in FILES] sprintf('%s/cycles.txt',FILE) using 1:2:3:4 with vectors nohead ls 1 lc 'grey' notitle , \
    for [FILE in FILES] sprintf('%s/tvals.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#226622' t "" 



==> plots/src/plot_tvalsc_merge <==
set key font ",8"
set key top left
set key Right
set key on
set yrange [-15:15]
set ytics 5

D = 9.765625
C=1
F = word(FILES,1)
X_MAX = real(system(sprintf("tail -n 1 %s/../elmo_str-eors_10k/cycles.txt  | cut -d ' ' -f1",F)))/C
set xrange [0:X_MAX]

load 'threshold.gp'
set xlabel "Cycle"
set ylabel "{/:Italic t}-test value"

plot for [FILE in FILES] sprintf('%s/../f030_str-eors_10k/tvals.txt',FILE) using ($0/D):1 with lines lt 1 lc rgb '#33AAEE' t "Device" , \
    for [FILE in FILES] sprintf('%s/../elmo_ori_str-eors_10k/tvals.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#AA88AA' t "ELMO" , \
    for [FILE in FILES] sprintf('%s/../elmo_str-eors_10k/tvals.txt',FILE) using ($0/C):1 with lines lt 1 lc rgb '#226622' lw 1.5 t "ELMO*" 


==> plots/src/temp.tex <==
\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Wed 06 Nov 2019 11:48:32 ACDT
\tikzset{every node/.append style={font={\fontsize{8.0pt}{9.6pt}\selectfont}}}
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.348,1.212)--(1.528,1.212);
\draw[gp path] (12.058,1.212)--(11.878,1.212);
\node[gp node right] at (1.201,1.212) {$-15$};
\draw[gp path] (1.348,1.820)--(1.528,1.820);
\draw[gp path] (12.058,1.820)--(11.878,1.820);
\node[gp node right] at (1.201,1.820) {$-12.5$};
\draw[gp path] (1.348,2.427)--(1.528,2.427);
\draw[gp path] (12.058,2.427)--(11.878,2.427);
\node[gp node right] at (1.201,2.427) {$-10$};
\draw[gp path] (1.348,3.035)--(1.528,3.035);
\draw[gp path] (12.058,3.035)--(11.878,3.035);
\node[gp node right] at (1.201,3.035) {$-7.5$};
\draw[gp path] (1.348,3.642)--(1.528,3.642);
\draw[gp path] (12.058,3.642)--(11.878,3.642);
\node[gp node right] at (1.201,3.642) {$-5$};
\draw[gp path] (1.348,4.250)--(1.528,4.250);
\draw[gp path] (12.058,4.250)--(11.878,4.250);
\node[gp node right] at (1.201,4.250) {$-2.5$};
\draw[gp path] (1.348,4.858)--(1.528,4.858);
\draw[gp path] (12.058,4.858)--(11.878,4.858);
\node[gp node right] at (1.201,4.858) {$0$};
\draw[gp path] (1.348,5.465)--(1.528,5.465);
\draw[gp path] (12.058,5.465)--(11.878,5.465);
\node[gp node right] at (1.201,5.465) {$2.5$};
\draw[gp path] (1.348,6.073)--(1.528,6.073);
\draw[gp path] (12.058,6.073)--(11.878,6.073);
\node[gp node right] at (1.201,6.073) {$5$};
\draw[gp path] (1.348,6.680)--(1.528,6.680);
\draw[gp path] (12.058,6.680)--(11.878,6.680);
\node[gp node right] at (1.201,6.680) {$7.5$};
\draw[gp path] (1.348,7.288)--(1.528,7.288);
\draw[gp path] (12.058,7.288)--(11.878,7.288);
\node[gp node right] at (1.201,7.288) {$10$};
\draw[gp path] (1.348,7.895)--(1.528,7.895);
\draw[gp path] (12.058,7.895)--(11.878,7.895);
\node[gp node right] at (1.201,7.895) {$12.5$};
\draw[gp path] (1.348,8.503)--(1.528,8.503);
\draw[gp path] (12.058,8.503)--(11.878,8.503);
\node[gp node right] at (1.201,8.503) {$15$};
\draw[gp path] (1.348,1.212)--(1.348,1.392);
\draw[gp path] (1.348,8.503)--(1.348,8.323);
\node[gp node center] at (1.348,0.821) {$0$};
\draw[gp path] (2.878,1.212)--(2.878,1.392);
\draw[gp path] (2.878,8.503)--(2.878,8.323);
\node[gp node center] at (2.878,0.821) {$2$};
\draw[gp path] (4.408,1.212)--(4.408,1.392);
\draw[gp path] (4.408,8.503)--(4.408,8.323);
\node[gp node center] at (4.408,0.821) {$4$};
\draw[gp path] (5.938,1.212)--(5.938,1.392);
\draw[gp path] (5.938,8.503)--(5.938,8.323);
\node[gp node center] at (5.938,0.821) {$6$};
\draw[gp path] (7.468,1.212)--(7.468,1.392);
\draw[gp path] (7.468,8.503)--(7.468,8.323);
\node[gp node center] at (7.468,0.821) {$8$};
\draw[gp path] (8.998,1.212)--(8.998,1.392);
\draw[gp path] (8.998,8.503)--(8.998,8.323);
\node[gp node center] at (8.998,0.821) {$10$};
\draw[gp path] (10.528,1.212)--(10.528,1.392);
\draw[gp path] (10.528,8.503)--(10.528,8.323);
\node[gp node center] at (10.528,0.821) {$12$};
\draw[gp path] (12.058,1.212)--(12.058,1.392);
\draw[gp path] (12.058,8.503)--(12.058,8.323);
\node[gp node center] at (12.058,0.821) {$14$};
\draw[gp path] (1.348,8.503)--(1.348,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (-0.101,4.857) {T-test value};
\node[gp node center,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (6.703,0.172) {Cycle};
\gpcolor{rgb color={0.753,0.753,0.753}}
\draw[gp path](1.348,8.503)--(1.348,1.212);
\draw[gp path](2.878,8.503)--(2.878,1.212);
\draw[gp path](3.643,8.503)--(3.643,1.212);
\draw[gp path](5.173,8.503)--(5.173,1.212);
\draw[gp path](5.938,8.503)--(5.938,1.212);
\draw[gp path](7.468,8.503)--(7.468,1.212);
\draw[gp path](8.998,8.503)--(8.998,1.212);
\draw[gp path](9.763,8.503)--(9.763,1.212);
\draw[gp path](11.293,8.503)--(11.293,1.212);
\draw[gp path](12.058,8.503)--(12.058,1.212);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.348,5.221)--(2.113,5.221)--(2.878,4.510)--(3.643,5.080)--(4.408,5.080)%
  --(5.173,3.201)--(5.938,3.201)--(6.703,4.011)--(7.468,4.976)--(8.233,4.976)--(8.998,1.964)%
  --(9.763,1.964)--(10.528,5.619)--(11.293,5.059)--(12.058,5.059);
\gpsetpointsize{0.40}
\gppoint{gp mark 2}{(1.348,5.221)}
\gppoint{gp mark 2}{(2.113,5.221)}
\gppoint{gp mark 2}{(2.878,4.510)}
\gppoint{gp mark 2}{(3.643,5.080)}
\gppoint{gp mark 2}{(4.408,5.080)}
\gppoint{gp mark 2}{(5.173,3.201)}
\gppoint{gp mark 2}{(5.938,3.201)}
\gppoint{gp mark 2}{(6.703,4.011)}
\gppoint{gp mark 2}{(7.468,4.976)}
\gppoint{gp mark 2}{(8.233,4.976)}
\gppoint{gp mark 2}{(8.998,1.964)}
\gppoint{gp mark 2}{(9.763,1.964)}
\gppoint{gp mark 2}{(10.528,5.619)}
\gppoint{gp mark 2}{(11.293,5.059)}
\gppoint{gp mark 2}{(12.058,5.059)}
\gpcolor{color=gp lt color border}
\draw[gp path] (1.348,8.503)--(1.348,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
\gpcolor{rgb color={1.000,0.000,0.000}}
\draw[gp path](1.348,5.951)--(12.058,5.951);
\draw[gp path](1.348,3.764)--(12.058,3.764);
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.348cm}{1.212cm}}{\pgfpoint{12.058cm}{8.503cm}}
\end{tikzpicture}
%% gnuplot variables


==> plots/src/xoodoo_plot_tvals_sample_merged <==

set yrange [0:50]
set xtics 0, 50000, 200000
#set xrange [0:10]
#set xtics ("0" 0, "2k" 20, "4k" 40, "6k" 60, "8k" 80, "10k" 100, "12k" 120, "14k" 140)
#set xtics ("0" 0, "2k" 200, "4k" 400, "6k" 600, "8k" 800, "10k" 1000, "12k" 1200, "14k" 1400, "16k" 1600, "18k" 1800, "20k" 2000)
#
set format x "%2.0s%c"
set label "Original Xoodoo implementation" at 10000,45
set arrow 3 from 104000,44 to 120000,40 head

set label "Fixed Xoodoo implementation" at 50700,18
set arrow 2 from 49500,15 to 20000,4 head

set arrow 1 from graph 0, first 4.5 to graph 1, first 4.5 nohead
set arrow 1 lc rgb "red"
set arrow 1 filled
set arrow 1 front 

set xlabel "Trace count"
set ylabel "Max {/:Italic t}-test value"



plot for [FILE in FILES] sprintf('%s/../f030_ttest_trend_xoodoo-check_200k/tvals_sample.txt',FILE)  using ($0 * 2500):1 with linespoints ps .01 lc "#00CC00" lw 1 t "" , \
    for [FILE in FILES] sprintf('%s/../f030_ttest_trend_xoodoo-fixed_200k/tvals_sample.txt',FILE)  using ($0 * 2500):1 with linespoints ps .01 lc "#0000FF"  lw 1 t ""


==> plots/traces_aligned.tex <==
%\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Mon 04 Nov 2019 15:30:52 ACDT
%\tikzset{every node/.append style={font={\fontsize{8.0pt}{9.6pt}\selectfont}}}
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,1.212)--(12.058,1.212);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,1.212)--(1.381,1.212);
\draw[gp path] (12.058,1.212)--(11.878,1.212);
\node[gp node right] at (1.054,1.212) {$-400$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,2.427)--(12.058,2.427);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,2.427)--(1.381,2.427);
\draw[gp path] (12.058,2.427)--(11.878,2.427);
\node[gp node right] at (1.054,2.427) {$-200$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,3.642)--(12.058,3.642);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,3.642)--(1.381,3.642);
\draw[gp path] (12.058,3.642)--(11.878,3.642);
\node[gp node right] at (1.054,3.642) {$0$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,4.858)--(12.058,4.858);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,4.858)--(1.381,4.858);
\draw[gp path] (12.058,4.858)--(11.878,4.858);
\node[gp node right] at (1.054,4.858) {$200$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,6.073)--(12.058,6.073);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,6.073)--(1.381,6.073);
\draw[gp path] (12.058,6.073)--(11.878,6.073);
\node[gp node right] at (1.054,6.073) {$400$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,7.288)--(12.058,7.288);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,7.288)--(1.381,7.288);
\draw[gp path] (12.058,7.288)--(11.878,7.288);
\node[gp node right] at (1.054,7.288) {$600$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,8.503)--(12.058,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,8.503)--(1.381,8.503);
\draw[gp path] (12.058,8.503)--(11.878,8.503);
\node[gp node right] at (1.054,8.503) {$800$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,1.212)--(1.201,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,1.212)--(1.201,1.392);
\draw[gp path] (1.201,8.503)--(1.201,8.323);
\node[gp node center] at (1.201,0.821) {$260$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (3.011,1.212)--(3.011,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (3.011,1.212)--(3.011,1.392);
\draw[gp path] (3.011,8.503)--(3.011,8.323);
\node[gp node center] at (3.011,0.821) {$265$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (4.820,1.212)--(4.820,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (4.820,1.212)--(4.820,1.392);
\draw[gp path] (4.820,8.503)--(4.820,8.323);
\node[gp node center] at (4.820,0.821) {$270$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (6.630,1.212)--(6.630,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (6.630,1.212)--(6.630,1.392);
\draw[gp path] (6.630,8.503)--(6.630,8.323);
\node[gp node center] at (6.630,0.821) {$275$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (8.439,1.212)--(8.439,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (8.439,1.212)--(8.439,1.392);
\draw[gp path] (8.439,8.503)--(8.439,8.323);
\node[gp node center] at (8.439,0.821) {$280$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (10.249,1.212)--(10.249,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (10.249,1.212)--(10.249,1.392);
\draw[gp path] (10.249,8.503)--(10.249,8.323);
\node[gp node center] at (10.249,0.821) {$285$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (12.058,1.212)--(12.058,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (12.058,1.212)--(12.058,1.392);
\draw[gp path] (12.058,8.503)--(12.058,8.323);
\node[gp node center] at (12.058,0.821) {$290$};
\draw[gp path] (1.201,8.503)--(1.201,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (-0.214,4.857) {Volatage (mV)};
\node[gp node center,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (6.629,0.172) {Timepoint (samples)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\gpsetlinewidth{0.20}
\draw[gp path] (1.201,2.640)--(1.563,1.874)--(1.925,4.930)--(2.287,7.324)--(2.649,5.793)%
  --(3.011,4.693)--(3.372,4.548)--(3.734,5.508)--(4.096,5.313)--(4.458,4.645)--(4.820,4.213)%
  --(5.182,3.551)--(5.544,6.225)--(5.906,5.459)--(6.268,4.499)--(6.630,3.071)--(6.991,3.071)%
  --(7.353,4.068)--(7.715,3.879)--(8.077,3.168)--(8.439,2.925)--(8.801,3.454)--(9.163,6.747)%
  --(9.525,4.450)--(9.887,3.503)--(10.249,3.023)--(10.610,3.685)--(10.972,4.311)--(11.334,3.831)%
  --(11.696,3.071)--(12.058,3.071);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.201,2.208)--(1.563,2.451)--(1.925,6.462)--(2.287,6.413)--(2.649,5.459)%
  --(3.011,4.645)--(3.372,4.833)--(3.734,6.127)--(4.096,5.216)--(4.458,4.402)--(4.820,3.642)%
  --(5.182,4.068)--(5.544,6.942)--(5.906,4.499)--(6.268,3.685)--(6.630,3.308)--(6.991,3.357)%
  --(7.353,4.450)--(7.715,3.977)--(8.077,3.168)--(8.439,2.737)--(8.801,4.548)--(9.163,5.508)%
  --(9.525,4.165)--(9.887,3.266)--(10.249,3.308)--(10.610,4.116)--(10.972,4.311)--(11.334,3.733)%
  --(11.696,3.308)--(12.058,3.600);
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (1.201,2.403)--(1.563,1.777)--(1.925,4.693)--(2.287,7.804)--(2.649,5.793)%
  --(3.011,5.076)--(3.372,4.785)--(3.734,5.125)--(4.096,5.550)--(4.458,4.742)--(4.820,3.733)%
  --(5.182,3.023)--(5.544,5.216)--(5.906,5.890)--(6.268,4.499)--(6.630,3.266)--(6.991,3.071)%
  --(7.353,3.733)--(7.715,3.879)--(8.077,3.308)--(8.439,2.688)--(8.801,3.168)--(9.163,6.942)%
  --(9.525,4.499)--(9.887,3.642)--(10.249,3.266)--(10.610,3.685)--(10.972,4.311)--(11.334,3.831)%
  --(11.696,3.217)--(12.058,2.543);
\gpcolor{rgb color={0.902,0.624,0.000}}
\draw[gp path] (1.201,2.306)--(1.563,1.923)--(1.925,4.596)--(2.287,7.658)--(2.649,5.745)%
  --(3.011,4.979)--(3.372,4.785)--(3.734,5.362)--(4.096,5.028)--(4.458,4.548)--(4.820,3.928)%
  --(5.182,3.266)--(5.544,5.216)--(5.906,5.793)--(6.268,4.645)--(6.630,3.551)--(6.991,3.168)%
  --(7.353,3.928)--(7.715,3.928)--(8.077,3.405)--(8.439,2.925)--(8.801,3.266)--(9.163,6.698)%
  --(9.525,4.833)--(9.887,3.928)--(10.249,3.357)--(10.610,3.551)--(10.972,4.359)--(11.334,3.928)%
  --(11.696,3.266)--(12.058,2.786);
\gpcolor{rgb color={0.941,0.894,0.259}}
\draw[gp path] (1.201,2.306)--(1.563,2.020)--(1.925,4.311)--(2.287,7.756)--(2.649,5.745)%
  --(3.011,5.076)--(3.372,4.548)--(3.734,5.216)--(4.096,5.459)--(4.458,4.785)--(4.820,3.782)%
  --(5.182,3.503)--(5.544,4.785)--(5.906,5.982)--(6.268,4.359)--(6.630,3.357)--(6.991,2.974)%
  --(7.353,3.782)--(7.715,3.879)--(8.077,3.405)--(8.439,2.834)--(8.801,3.266)--(9.163,6.607)%
  --(9.525,4.693)--(9.887,4.019)--(10.249,3.266)--(10.610,3.308)--(10.972,4.262)--(11.334,3.879)%
  --(11.696,3.357)--(12.058,2.925);
\gpcolor{rgb color={0.000,0.447,0.698}}
\draw[gp path] (1.201,2.591)--(1.563,1.923)--(1.925,5.647)--(2.287,6.893)--(2.649,5.793)%
  --(3.011,4.548)--(3.372,4.645)--(3.734,5.647)--(4.096,5.313)--(4.458,4.402)--(4.820,3.831)%
  --(5.182,3.733)--(5.544,7.081)--(5.906,5.028)--(6.268,4.165)--(6.630,3.168)--(6.991,3.168)%
  --(7.353,4.165)--(7.715,3.831)--(8.077,3.308)--(8.439,2.786)--(8.801,4.068)--(9.163,6.225)%
  --(9.525,4.311)--(9.887,3.023)--(10.249,3.023)--(10.610,3.977)--(10.972,4.359)--(11.334,3.642)%
  --(11.696,3.454)--(12.058,3.308);
\gpcolor{rgb color={0.898,0.118,0.063}}
\draw[gp path] (1.201,2.883)--(1.563,2.257)--(1.925,4.499)--(2.287,7.658)--(2.649,5.696)%
  --(3.011,4.979)--(3.372,4.645)--(3.734,5.216)--(4.096,5.410)--(4.458,4.693)--(4.820,4.213)%
  --(5.182,3.308)--(5.544,4.596)--(5.906,5.890)--(6.268,4.499)--(6.630,3.120)--(6.991,2.974)%
  --(7.353,3.600)--(7.715,3.928)--(8.077,3.503)--(8.439,3.120)--(8.801,3.120)--(9.163,6.462)%
  --(9.525,4.693)--(9.887,3.977)--(10.249,2.883)--(10.610,3.217)--(10.972,4.311)--(11.334,3.879)%
  --(11.696,3.266)--(12.058,2.834);
\gpcolor{rgb color={0.000,0.000,0.000}}
\draw[gp path] (1.201,1.971)--(1.563,1.637)--(1.925,5.599)--(2.287,6.316)--(2.649,5.508)%
  --(3.011,4.645)--(3.372,4.742)--(3.734,5.647)--(4.096,4.742)--(4.458,4.019)--(4.820,3.405)%
  --(5.182,3.600)--(5.544,6.844)--(5.906,4.742)--(6.268,3.879)--(6.630,3.266)--(6.991,3.168)%
  --(7.353,3.879)--(7.715,3.266)--(8.077,2.925)--(8.439,2.403)--(8.801,3.551)--(9.163,5.550)%
  --(9.525,4.262)--(9.887,3.357)--(10.249,3.023)--(10.610,3.831)--(10.972,4.019)--(11.334,3.357)%
  --(11.696,2.925)--(12.058,2.974);
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (1.201,2.208)--(1.563,1.637)--(1.925,5.028)--(2.287,6.942)--(2.649,5.550)%
  --(3.011,4.882)--(3.372,4.785)--(3.734,5.410)--(4.096,4.833)--(4.458,4.359)--(4.820,3.685)%
  --(5.182,3.503)--(5.544,6.510)--(5.906,5.167)--(6.268,4.402)--(6.630,3.503)--(6.991,3.168)%
  --(7.353,3.879)--(7.715,3.831)--(8.077,3.454)--(8.439,2.786)--(8.801,3.454)--(9.163,6.607)%
  --(9.525,4.402)--(9.887,3.600)--(10.249,3.071)--(10.610,3.831)--(10.972,4.116)--(11.334,3.928)%
  --(11.696,3.217)--(12.058,2.688);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.201,2.160)--(1.563,1.589)--(1.925,4.645)--(2.287,6.893)--(2.649,5.599)%
  --(3.011,4.742)--(3.372,4.499)--(3.734,5.265)--(4.096,5.125)--(4.458,4.311)--(4.820,3.600)%
  --(5.182,3.217)--(5.544,5.745)--(5.906,5.076)--(6.268,4.499)--(6.630,3.405)--(6.991,2.974)%
  --(7.353,3.782)--(7.715,3.733)--(8.077,3.071)--(8.439,2.451)--(8.801,3.120)--(9.163,6.413)%
  --(9.525,4.359)--(9.887,3.600)--(10.249,3.023)--(10.610,3.551)--(10.972,4.262)--(11.334,3.600)%
  --(11.696,2.834)--(12.058,2.543);
\gpcolor{color=gp lt color border}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,8.503)--(1.201,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.201cm}{1.212cm}}{\pgfpoint{12.058cm}{8.503cm}}
%\end{tikzpicture}
%% gnuplot variables


==> plots/traces_notaligned.tex <==
%\begin{tikzpicture}[gnuplot]
%% generated with GNUPLOT 5.2p2 (Lua 5.3; terminal rev. 99, script rev. 102)
%% Mon 04 Nov 2019 15:30:43 ACDT
%\tikzset{every node/.append style={font={\fontsize{8.0pt}{9.6pt}\selectfont}}}
\path (0.000,0.000) rectangle (12.500,8.750);
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,1.212)--(12.058,1.212);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,1.212)--(1.381,1.212);
\draw[gp path] (12.058,1.212)--(11.878,1.212);
\node[gp node right] at (1.054,1.212) {$-400$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,2.427)--(12.058,2.427);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,2.427)--(1.381,2.427);
\draw[gp path] (12.058,2.427)--(11.878,2.427);
\node[gp node right] at (1.054,2.427) {$-200$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,3.642)--(12.058,3.642);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,3.642)--(1.381,3.642);
\draw[gp path] (12.058,3.642)--(11.878,3.642);
\node[gp node right] at (1.054,3.642) {$0$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,4.858)--(12.058,4.858);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,4.858)--(1.381,4.858);
\draw[gp path] (12.058,4.858)--(11.878,4.858);
\node[gp node right] at (1.054,4.858) {$200$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,6.073)--(12.058,6.073);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,6.073)--(1.381,6.073);
\draw[gp path] (12.058,6.073)--(11.878,6.073);
\node[gp node right] at (1.054,6.073) {$400$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,7.288)--(12.058,7.288);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,7.288)--(1.381,7.288);
\draw[gp path] (12.058,7.288)--(11.878,7.288);
\node[gp node right] at (1.054,7.288) {$600$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,8.503)--(12.058,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,8.503)--(1.381,8.503);
\draw[gp path] (12.058,8.503)--(11.878,8.503);
\node[gp node right] at (1.054,8.503) {$800$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (1.201,1.212)--(1.201,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,1.212)--(1.201,1.392);
\draw[gp path] (1.201,8.503)--(1.201,8.323);
\node[gp node center] at (1.201,0.821) {$260$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (3.011,1.212)--(3.011,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (3.011,1.212)--(3.011,1.392);
\draw[gp path] (3.011,8.503)--(3.011,8.323);
\node[gp node center] at (3.011,0.821) {$265$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (4.820,1.212)--(4.820,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (4.820,1.212)--(4.820,1.392);
\draw[gp path] (4.820,8.503)--(4.820,8.323);
\node[gp node center] at (4.820,0.821) {$270$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (6.630,1.212)--(6.630,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (6.630,1.212)--(6.630,1.392);
\draw[gp path] (6.630,8.503)--(6.630,8.323);
\node[gp node center] at (6.630,0.821) {$275$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (8.439,1.212)--(8.439,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (8.439,1.212)--(8.439,1.392);
\draw[gp path] (8.439,8.503)--(8.439,8.323);
\node[gp node center] at (8.439,0.821) {$280$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (10.249,1.212)--(10.249,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (10.249,1.212)--(10.249,1.392);
\draw[gp path] (10.249,8.503)--(10.249,8.323);
\node[gp node center] at (10.249,0.821) {$285$};
\gpcolor{color=gp lt color axes}
\gpsetlinetype{gp lt axes}
\gpsetdashtype{gp dt axes}
\gpsetlinewidth{0.50}
\draw[gp path] (12.058,1.212)--(12.058,8.503);
\gpcolor{color=gp lt color border}
\gpsetlinetype{gp lt border}
\gpsetdashtype{gp dt solid}
\gpsetlinewidth{1.00}
\draw[gp path] (12.058,1.212)--(12.058,1.392);
\draw[gp path] (12.058,8.503)--(12.058,8.323);
\node[gp node center] at (12.058,0.821) {$290$};
\draw[gp path] (1.201,8.503)--(1.201,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
\node[gp node center,rotate=-270,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (-0.214,4.857) {Volatage (mV)};
\node[gp node center,font={\fontsize{16.0pt}{19.2pt}\selectfont}] at (6.629,0.172) {Timepoint (samples)};
\gpcolor{rgb color={0.580,0.000,0.827}}
\gpsetlinewidth{0.20}
\draw[gp path] (1.201,2.306)--(1.563,1.686)--(1.925,5.216)--(2.287,6.844)--(2.649,5.265)%
  --(3.011,4.499)--(3.372,4.450)--(3.734,5.550)--(4.096,5.076)--(4.458,4.499)--(4.820,3.733)%
  --(5.182,3.600)--(5.544,6.656)--(5.906,4.930)--(6.268,3.831)--(6.630,3.120)--(6.991,2.925)%
  --(7.353,3.831)--(7.715,3.551)--(8.077,3.217)--(8.439,2.640)--(8.801,3.551)--(9.163,6.079)%
  --(9.525,4.019)--(9.887,3.071)--(10.249,2.737)--(10.610,3.405)--(10.972,4.068)--(11.334,3.879)%
  --(11.696,3.266)--(12.058,2.883);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.201,2.591)--(1.563,1.923)--(1.925,4.213)--(2.287,7.756)--(2.649,6.176)%
  --(3.011,5.362)--(3.372,4.693)--(3.734,5.362)--(4.096,5.745)--(4.458,4.742)--(4.820,3.879)%
  --(5.182,3.120)--(5.544,4.402)--(5.906,6.079)--(6.268,4.596)--(6.630,3.308)--(6.991,3.217)%
  --(7.353,3.977)--(7.715,4.165)--(8.077,3.308)--(8.439,2.925)--(8.801,3.120)--(9.163,6.364)%
  --(9.525,4.742)--(9.887,4.213)--(10.249,3.405)--(10.610,3.642)--(10.972,4.402)--(11.334,4.019)%
  --(11.696,3.308)--(12.058,3.023);
\gpcolor{rgb color={0.337,0.706,0.914}}
\draw[gp path] (1.201,2.257)--(1.563,3.831)--(1.925,7.178)--(2.287,5.890)--(2.649,5.410)%
  --(3.011,4.833)--(3.372,5.028)--(3.734,5.842)--(4.096,4.930)--(4.458,4.359)--(4.820,3.685)%
  --(5.182,4.019)--(5.544,6.364)--(5.906,4.402)--(6.268,3.551)--(6.630,3.071)--(6.991,3.168)%
  --(7.353,4.213)--(7.715,3.782)--(8.077,3.168)--(8.439,2.834)--(8.801,5.167)--(9.163,5.076)%
  --(9.525,4.262)--(9.887,3.266)--(10.249,2.974)--(10.610,4.402)--(10.972,4.262)--(11.334,3.782)%
  --(11.696,3.071)--(12.058,3.551);
\gpcolor{rgb color={0.902,0.624,0.000}}
\draw[gp path] (1.201,2.640)--(1.563,1.874)--(1.925,4.930)--(2.287,7.324)--(2.649,5.793)%
  --(3.011,4.693)--(3.372,4.548)--(3.734,5.508)--(4.096,5.313)--(4.458,4.645)--(4.820,4.213)%
  --(5.182,3.551)--(5.544,6.225)--(5.906,5.459)--(6.268,4.499)--(6.630,3.071)--(6.991,3.071)%
  --(7.353,4.068)--(7.715,3.879)--(8.077,3.168)--(8.439,2.925)--(8.801,3.454)--(9.163,6.747)%
  --(9.525,4.450)--(9.887,3.503)--(10.249,3.023)--(10.610,3.685)--(10.972,4.311)--(11.334,3.831)%
  --(11.696,3.071)--(12.058,3.071);
\gpcolor{rgb color={0.941,0.894,0.259}}
\draw[gp path] (1.201,2.208)--(1.563,2.451)--(1.925,6.462)--(2.287,6.413)--(2.649,5.459)%
  --(3.011,4.645)--(3.372,4.833)--(3.734,6.127)--(4.096,5.216)--(4.458,4.402)--(4.820,3.642)%
  --(5.182,4.068)--(5.544,6.942)--(5.906,4.499)--(6.268,3.685)--(6.630,3.308)--(6.991,3.357)%
  --(7.353,4.450)--(7.715,3.977)--(8.077,3.168)--(8.439,2.737)--(8.801,4.548)--(9.163,5.508)%
  --(9.525,4.165)--(9.887,3.266)--(10.249,3.308)--(10.610,4.116)--(10.972,4.311)--(11.334,3.733)%
  --(11.696,3.308)--(12.058,3.600);
\gpcolor{rgb color={0.000,0.447,0.698}}
\draw[gp path] (1.201,1.777)--(1.563,4.693)--(1.925,7.804)--(2.287,5.793)--(2.649,5.076)%
  --(3.011,4.785)--(3.372,5.125)--(3.734,5.550)--(4.096,4.742)--(4.458,3.733)--(4.820,3.023)%
  --(5.182,5.216)--(5.544,5.890)--(5.906,4.499)--(6.268,3.266)--(6.630,3.071)--(6.991,3.733)%
  --(7.353,3.879)--(7.715,3.308)--(8.077,2.688)--(8.439,3.168)--(8.801,6.942)--(9.163,4.499)%
  --(9.525,3.642)--(9.887,3.266)--(10.249,3.685)--(10.610,4.311)--(10.972,3.831)--(11.334,3.217)%
  --(11.696,2.543)--(12.058,4.311);
\gpcolor{rgb color={0.898,0.118,0.063}}
\draw[gp path] (1.201,1.923)--(1.563,4.596)--(1.925,7.658)--(2.287,5.745)--(2.649,4.979)%
  --(3.011,4.785)--(3.372,5.362)--(3.734,5.028)--(4.096,4.548)--(4.458,3.928)--(4.820,3.266)%
  --(5.182,5.216)--(5.544,5.793)--(5.906,4.645)--(6.268,3.551)--(6.630,3.168)--(6.991,3.928)%
  --(7.353,3.928)--(7.715,3.405)--(8.077,2.925)--(8.439,3.266)--(8.801,6.698)--(9.163,4.833)%
  --(9.525,3.928)--(9.887,3.357)--(10.249,3.551)--(10.610,4.359)--(10.972,3.928)--(11.334,3.266)%
  --(11.696,2.786)--(12.058,4.262);
\gpcolor{rgb color={0.000,0.000,0.000}}
\draw[gp path] (1.201,2.306)--(1.563,2.020)--(1.925,4.311)--(2.287,7.756)--(2.649,5.745)%
  --(3.011,5.076)--(3.372,4.548)--(3.734,5.216)--(4.096,5.459)--(4.458,4.785)--(4.820,3.782)%
  --(5.182,3.503)--(5.544,4.785)--(5.906,5.982)--(6.268,4.359)--(6.630,3.357)--(6.991,2.974)%
  --(7.353,3.782)--(7.715,3.879)--(8.077,3.405)--(8.439,2.834)--(8.801,3.266)--(9.163,6.607)%
  --(9.525,4.693)--(9.887,4.019)--(10.249,3.266)--(10.610,3.308)--(10.972,4.262)--(11.334,3.879)%
  --(11.696,3.357)--(12.058,2.925);
\gpcolor{rgb color={0.580,0.000,0.827}}
\draw[gp path] (1.201,2.591)--(1.563,1.923)--(1.925,5.647)--(2.287,6.893)--(2.649,5.793)%
  --(3.011,4.548)--(3.372,4.645)--(3.734,5.647)--(4.096,5.313)--(4.458,4.402)--(4.820,3.831)%
  --(5.182,3.733)--(5.544,7.081)--(5.906,5.028)--(6.268,4.165)--(6.630,3.168)--(6.991,3.168)%
  --(7.353,4.165)--(7.715,3.831)--(8.077,3.308)--(8.439,2.786)--(8.801,4.068)--(9.163,6.225)%
  --(9.525,4.311)--(9.887,3.023)--(10.249,3.023)--(10.610,3.977)--(10.972,4.359)--(11.334,3.642)%
  --(11.696,3.454)--(12.058,3.308);
\gpcolor{rgb color={0.000,0.620,0.451}}
\draw[gp path] (1.201,2.257)--(1.563,4.499)--(1.925,7.658)--(2.287,5.696)--(2.649,4.979)%
  --(3.011,4.645)--(3.372,5.216)--(3.734,5.410)--(4.096,4.693)--(4.458,4.213)--(4.820,3.308)%
  --(5.182,4.596)--(5.544,5.890)--(5.906,4.499)--(6.268,3.120)--(6.630,2.974)--(6.991,3.600)%
  --(7.353,3.928)--(7.715,3.503)--(8.077,3.120)--(8.439,3.120)--(8.801,6.462)--(9.163,4.693)%
  --(9.525,3.977)--(9.887,2.883)--(10.249,3.217)--(10.610,4.311)--(10.972,3.879)--(11.334,3.266)%
  --(11.696,2.834)--(12.058,3.782);
\gpcolor{color=gp lt color border}
\gpsetlinewidth{1.00}
\draw[gp path] (1.201,8.503)--(1.201,1.212)--(12.058,1.212)--(12.058,8.503)--cycle;
%% coordinates of the plot area
\gpdefrectangularnode{gp plot 1}{\pgfpoint{1.201cm}{1.212cm}}{\pgfpoint{12.058cm}{8.503cm}}
%\end{tikzpicture}
%% gnuplot variables


==> t-gnuplot-lua-tikz.tex <==
%%
%%  ConTeXt wrapper for gnuplot-tikz style file
%%
\usemodule[tikz]

\usetikzlibrary[arrows,patterns,plotmarks,backgrounds]

\edef\tikzatcode{\the\catcode`\@}
\edef\tikzbarcode{\the\catcode`\|}
\edef\tikzexclaimcode{\the\catcode`\!}
\catcode`\@=11
\catcode`\|=12
\catcode`\!=12

\input gnuplot-lua-tikz-common.tex

\catcode`\@=\tikzatcode
\catcode`\|=\tikzbarcode
\catcode`\!=\tikzexclaimcode

\endinput

